On Near-Far-Field Boundaries in Wireless Systems

Near-field (NF) multi-antenna wireless communication and sensing have attracted growing research interest in recent years. A core question in this area is how to determine whether a wireless system is operating in the NF or far-field (FF) region. In this work, we propose a framework grounded in Maxwell's equations to analyze the transition region between the NF and FF, following the IEEE definition that specifies where the NF ends and the FF begins. Using this framework, we (i) compare a variety of traditional and recently introduced single-letter distance thresholds, often referred to as near-far-field boundaries, and (ii) conduct numerical experiments with both single- and multi-antenna wireless systems and with analytical models as well as full-wave electromagnetic simulations. Our results indicate that all of the considered single-letter distance thresholds are insufficient to predict the transition region between the NF and FF regions. Moreover, we highlight several important caveats associated with frequently (and recently) used NF and FF concepts.

==> sty/26XX_NFFB-macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Color Palette:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{sty/eth-colours}

% corporate design colors
\colorlet{blue}{eth_blue}
\colorlet{blue_10}{eth_blue_10}
\colorlet{blue_20}{eth_blue_20}
\colorlet{blue_60}{eth_blue_60}
\colorlet{blue_80}{eth_blue_80}
\colorlet{blue_120}{eth_blue_120}

\colorlet{petrol_120}{eth_petrol_120}
\colorlet{petrol}{eth_petrol}
\colorlet{petrol_10}{eth_petrol_10}
\colorlet{petrol_20}{eth_petrol_20}

\colorlet{green_120}{eth_green_120}
\colorlet{green}{eth_green}
\colorlet{green_10}{eth_green_10}
\colorlet{green_60}{eth_green_60}
\colorlet{green_80}{eth_green_80}
\colorlet{green_120}{eth_green_120}

\colorlet{bronze_120}{eth_bronze_120}
\colorlet{bronze}{eth_bronze}
\colorlet{bronze_80}{eth_bronze_80}
\colorlet{bronze_10}{eth_bronze_10}

\colorlet{red_120}{eth_red_120}
\colorlet{red}{eth_red}
\colorlet{red_80}{eth_red_80}
\colorlet{red_10}{eth_red_10}

\colorlet{purple_120}{eth_purple_120}
\colorlet{purple}{eth_purple}
\colorlet{purple_80}{eth_purple_80}
\colorlet{purple_20}{eth_purple_20}
\colorlet{purple_10}{eth_purple_10}


\colorlet{black}{eth_black}
\colorlet{black_light}{eth_black_light}
\colorlet{black_60}{eth_black_60}
\colorlet{black_light_48}{eth_black_light_48}
\colorlet{black_light_20}{eth_black_light_20}
\colorlet{grey_120}{eth_grey_120}
\colorlet{grey}{eth_grey}
\colorlet{grey_10}{eth_grey_10}
\colorlet{grey_05}{eth_grey_05}

\definecolor{pink}{RGB}{214,82,130}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Tikz Macros:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclarepatternformonly{south east lines my}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{5pt}{5pt}}{\pgfqpoint{5pt}{5pt}}{
    \pgfsetlinewidth{0.5pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{5pt}}
    \pgfpathlineto{\pgfqpoint{5pt}{0pt}}
    \pgfpathmoveto{\pgfqpoint{.2pt}{-.2pt}}
    \pgfpathlineto{\pgfqpoint{-.2pt}{.2pt}}
    \pgfpathmoveto{\pgfqpoint{5.2pt}{4.8pt}}
    \pgfpathlineto{\pgfqpoint{4.8pt}{5.2pt}}
    \pgfusepath{stroke}}
    
\pgfdeclarepatternformonly{horizontal lines my}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{3.54pt}{3.54pt}}{\pgfqpoint{3.54pt}{3.54pt}}{
    \pgfsetlinewidth{0.5pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{2pt}}
    \pgfpathlineto{\pgfqpoint{3.54pt}{2pt}}
    \pgfusepath{stroke}}

\pgfdeclarepatternformonly{diagonal behind text}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{15pt}{15pt}}{\pgfqpoint{15pt}{15pt}}{
    \pgfsetlinewidth{0.7pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
    \pgfpathlineto{\pgfqpoint{15pt}{15pt}}
    \pgfpathmoveto{\pgfqpoint{14.8pt}{-.2pt}}
    \pgfpathlineto{\pgfqpoint{15.2pt}{.2pt}}
    \pgfpathmoveto{\pgfqpoint{-.2pt}{14.8pt}}
    \pgfpathlineto{\pgfqpoint{.2pt}{15.2pt}}
    \pgfusepath{stroke}}

\pgfdeclarepatternformonly{diagonal pattern node}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{3pt}{3pt}}{\pgfqpoint{3pt}{3pt}}{
    \pgfsetlinewidth{0.7pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
    \pgfpathlineto{\pgfqpoint{3pt}{3pt}}
    \pgfpathmoveto{\pgfqpoint{2.8pt}{-.2pt}}
    \pgfpathlineto{\pgfqpoint{3.2pt}{.2pt}}
    \pgfpathmoveto{\pgfqpoint{-.2pt}{2.8pt}}
    \pgfpathlineto{\pgfqpoint{.2pt}{3.2pt}}
    \pgfusepath{stroke}}

\def\centerOfC at (#1,#2){
    \draw  [shift={(#1,#2)}, rotate=-45,line width=0pt, fill=white, color=white, anchor=center] (-.27,-.27) rectangle (.27,.27);
    \draw  [shift={(#1,#2)}, rotate=-45,line width=0pt, fill=white, color=white, anchor=center] (-.3,-.15) rectangle (.3,.15);

    
    \draw  [shift={(#1,#2)},line width=0.3pt, fill=white] (0,0) ellipse (0.16 and 0.16);
    \draw [shift={(#1,#2)},line width=0.3pt, color=black] (-0.2,0) -- (0.2,0);
    \draw [shift={(#1,#2)},line width=0.3pt, color=black] (0,-0.2) -- (0,0.2);
    \draw [shift={(#1,#2)},line width=0.3pt, color=black, fill=black]  (0,0) -- (0:0.16) arc (0:90:.16) -- cycle;
    \draw [shift={(#1,#2)},line width=0.3pt, color=black, fill=black]  (0,0) -- (180:0.16) arc (180:90+180:.16) -- cycle;
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Operators:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator{\diag}{diag}			        % diag matrix
\DeclareMathOperator{\Ex}{\mathbb{E}}		        % expectation operator
\newcommand{\T}[0]{\mathsf{T}}                      % transpose
\newcommand{\He}[0]{\mathsf{H}}                     % hermitian
\DeclareMathOperator*{\argmin}{arg\,min}            % argmax
\DeclareMathOperator*{\maximize}{maximize}          % maximize     
\newcommand\smallO{                                 % small o 
  \mathchoice
    {{\scriptstyle\mathcal{O}}}
    {{\scriptstyle\mathcal{O}}}
    {{\scriptscriptstyle\mathcal{O}}}
    {\scalebox{.7}{$\scriptscriptstyle\mathcal{O}$}}
  }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Font Macros:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\up}[1]{{\textnormal{#1}}}              % subscripts

\newcommand{\mat}[1]{{\bm{\mathbf{#1}}}}            % matrices
\newcommand{\vect}[1]{{\bm{\mathbf{#1}}}}           % vectors
\newcommand{\oper}[1]{\mathbb{#1}}                  % operator

\newcommand{\phs}[1]{{\mathsf{#1}}}  % phasor scalar
\newcommand{\phv}[1]{{\bm{\mathsf{#1}}}} % phasor vector



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Fancy Ref Stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand*{\fancyrefapplabelprefix}{app}		% Appendix
\newcommand*{\fancyrefthmlabelprefix}{thm}		% Theorem
\newcommand*{\fancyrefdefilabelprefix}{defi}    % Definition
\newcommand*{\fancyrefproplabelprefix}{prop}	% Proposition
\newcommand*{\fancyrefalglabelprefix}{alg}		% Algorithm
\newcommand*{\fancyrefasmlabelprefix}{asm}		% Assumption
\newcommand*{\fancyrefremlabelprefix}{rem}		% Remark
\newcommand*{\fancyrefwarlabelprefix}{war}		% Warning 


% label names
\frefformat{vario}{\fancyrefthmlabelprefix}{Theorem~#1}
\frefformat{vario}{\fancyrefdefilabelprefix}{Definition~#1}
\frefformat{vario}{\fancyreffiglabelprefix}{Figure~#1}
\frefformat{vario}{\fancyrefapplabelprefix}{Appendix~#1}
\frefformat{vario}{\fancyrefeqlabelprefix}{(#1)}
\frefformat{vario}{\fancyrefproplabelprefix}{Proposition~#1}
\frefformat{vario}{\fancyrefalglabelprefix}{Algorithm~#1}
\frefformat{vario}{\fancyrefasmlabelprefix}{Assumption~#1}
\frefformat{vario}{\fancyrefremlabelprefix}{Remark~#1}
\frefformat{vario}{\fancyrefwarlabelprefix}{Warning Note~#1}
\frefformat{vario}{\fancyrefseclabelprefix}{Section~#1}
\frefformat{vario}{\fancyreftablabelprefix}{Table~#1}

%-------  Colors -------%
\newcommand{\red}[1]{{\color{red}{#1}}} 
\newcommand{\blue}[1]{{\color{blue}{#1}}}
\newcommand{\green}[1]{{\color{green}{#1}}} 
\newcommand{\yellow}[1]{{\color{yellow}{#1}}} 
\newcommand{\orange}[1]{{\color{orange}{#1}}} 


==> sty/eth-colours.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% ETH Zürich's Corporate Design Colours
%%
%% Alexander Stutz (alstutz@iis.ee.ethz.ch)
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% corporate design colours
\definecolor{eth_blue}{RGB}{33, 92, 175}
\definecolor{eth_blue_10}{RGB}{233, 239, 247}
\definecolor{eth_blue_20}{RGB}{211, 222, 239}
\definecolor{eth_blue_60}{RGB}{122, 157, 207}
\definecolor{eth_blue_80}{RGB}{77, 125, 191}
\definecolor{eth_blue_120}{RGB}{8, 64, 126}

\definecolor{eth_petrol_120}{RGB}{0, 89, 109}
\definecolor{eth_petrol}{RGB}{0, 120, 148}
\definecolor{eth_petrol_10}{RGB}{231, 244, 247}
\definecolor{eth_petrol_20}{RGB}{204, 228, 234}

\definecolor{eth_green_120}{RGB}{60, 81, 30}
\definecolor{eth_green}{RGB}{98, 115, 19}
\definecolor{eth_green_10}{RGB}{239, 241, 231}
\definecolor{eth_green_60}{RGB}{161, 171, 113}
\definecolor{eth_green_80}{RGB}{129, 143, 66}
\definecolor{eth_green_120}{RGB}{54, 82, 19}

\definecolor{eth_bronze_120}{RGB}{107, 80, 31}
\definecolor{eth_bronze}{RGB}{142, 103, 19}
\definecolor{eth_bronze_80}{RGB}{165, 133, 66}
\definecolor{eth_bronze_10}{RGB}{244, 240, 231}

\definecolor{eth_red_120}{RGB}{150, 39, 45}
\definecolor{eth_red}{RGB}{183, 53, 45}
\definecolor{eth_red_80}{RGB}{197, 93, 87}
\definecolor{eth_red_10}{RGB}{248, 235, 234}

\definecolor{eth_purple_120}{RGB}{140, 10, 89}
\definecolor{eth_purple}{RGB}{167, 17, 122}
\definecolor{eth_purple_80}{RGB}{183, 59, 146}
\definecolor{eth_purple_20}{RGB}{239, 208, 227}
\definecolor{eth_purple_10}{RGB}{248, 232, 243}


\definecolor{eth_grey_120}{RGB}{87, 87, 87}
\definecolor{eth_grey}{RGB}{111, 111, 111}
\definecolor{eth_grey_10}{RGB}{241, 241, 241}


% black and shades of grey
% (for non-white background check required opacity online)
\definecolor{eth_black}{RGB}{0, 0, 0}
\definecolor{eth_black_light}{RGB}{34, 34, 34}
\definecolor{eth_black_60}{RGB}{102, 102, 102}
\definecolor{eth_black_light_48}{RGB}{149,149,149}
\definecolor{eth_black_light_20}{RGB}{211, 211, 211}
\definecolor{eth_grey_10}{RGB}{241, 241, 241}
\definecolor{eth_grey_05}{RGB}{246, 246, 246}





